HiT-DVAE: Human Motion Generation via Hierarchical Transformer Dynamical VAE

Studies on the automatic processing of 3D human pose data have flourished in the recent past. In this paper, we are interested in the generation of plausible and diverse future human poses following an observed 3D pose sequence. Current methods address this problem by injecting random variables from a single latent space into a deterministic motion prediction framework, which precludes the inherent multi-modality in human motion generation. In addition, previous works rarely explore the use of attention to select which frames are to be used to inform the generation process up to our knowledge. To overcome these limitations, we propose Hierarchical Transformer Dynamical Variational Autoencoder, HiT-DVAE, which implements auto-regressive generation with transformer-like attention mechanisms. HiT-DVAE simultaneously learns the evolution of data and latent space distribution with time correlated probabilistic dependencies, thus enabling the generative model to learn a more complex and time-varying latent space as well as diverse and realistic human motions. Furthermore, the auto-regressive generation brings more flexibility on observation and prediction, i.e. one can have any length of observation and predict arbitrary large sequences of poses with a single pre-trained model. We evaluate the proposed method on HumanEva-I and Human3.6M with various evaluation methods, and outperform the state-of-the-art methods on most of the metrics.

==> fig_pipeline.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/pipeline_v2.4.png} %{figures/pipeline_v2.png}
    \caption{Pipeline. HIT-DVAE Encoder take the observed sequence $\myx_{1:T}$ as input to estimate the posterior distribution of the time-dependent latent variables  $\myz_{1:T}$ and time-independent latent variable $\myw$. Then the Decoder will reconstruct the data and prior of $\myz$. To avoid learning a prior model on $\myx_0$ and $\myz_0$, we start generation at frame 2, this will facilitate the training and do not affect the latter motion generation.}
    \label{fig:TransDVAE}
\end{figure*}

==> tab_data_aug.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Augmentation for motion prediction on \textbf{HumanEva-I}. Average result, 10 frames. in mm. \wen{TODO: add in supp: different prediction length / best-medium augmentation}}
\label{table:tab_aug}
\resizebox{0.8\textwidth}{!}{\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{l|cccc|cccc}
\hline%\noalign{\smallskip}
 & \multicolumn{4}{c|}{HumanEva-I} & \multicolumn{4}{c}{Human3.6M} \\
 \hline
 & w.o. aug & DLow & gsps & HiT-DVAE & w.o. aug & DLow & gsps & HiT-DVAE\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
LTD & 26.51 & &  & & & & &\\
Hisrep & 26.53 & & & & & & &\\
\hline
\end{tabular}}}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}



